Semantic Analysis of Subexponential Modalities in Distributive Non-commutative Linear Logic

In this paper, we consider the full Lambek calculus enriched with subexponential modalities in a distributive setting. We show that the distributive Lambek calculus with subexponentials is complete with respect to its Kripke frames via canonical extensions. In this approach, we consider subexponentials as S4-like modalities and each modality is interpreted with a reflexive and transitive relation similarly to usual Kripke semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{60}
\providecommand{\publicationstatus}{M. Moortgat and M. Sadrzadeh (Eds.): Modalities in substructural logics.\\
Applications at the interfaces of logic, language and computation (AMSLO 2023).\\
EPTCS 381, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.381.7}{10.4204/EPTCS.381.7}}

